Understanding Open Source Serverless Platforms: Design Considerations and Performance

Serverless computing is increasingly popular because of the promise of lower cost and the convenience it provides to users who do not need to focus on server management. This has resulted in the availability of a number of proprietary and open-source serverless solutions. We seek to understand how the performance of serverless computing depends on a number of design issues using several popular open-source serverless platforms. We identify the idiosyncrasies affecting performance (throughput and latency) for different open-source serverless platforms. Further, we observe that just having either resource-based (CPU and memory) or workload-based (request per second (RPS) or concurrent requests) auto-scaling is inadequate to address the needs of the serverless platforms.

==> Serverless_measurement-12 copy/plots/eval1_plots.tex <==
\hide{
\begin{figure*}[htb!]
\begin{subfigure}{.5\textwidth}
    \centering
    \includegraphics[width=3.2in, trim=0.01cm 0.01cm 0.01cm 0.01cm, clip=true]{plots/access_mode_rps_barplot.pdf}
    \vspace{-3mm}
    \caption{Throughput in requests/second.}
    \label{fig:ThroughputDiffModes}
    % \vspace{-4mm}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
	\centering
	\includegraphics[width=3.4in, trim=0.01cm 0.01cm 0.01cm 0.01cm, clip=true]{plots/boxplot_configuration.pdf}
    \vspace{-3mm}
    \caption{Latency in ms.}
    \label{fig:LatencyDiffModes}
    \vspace{-6mm}
\end{subfigure}
\caption{Throughput and latency for different methods of exporting the services for different serverless platforms.}
\label{fig:DiffModes}
\end{figure*}
}
\hide{
\begin{figure}[htb!]
\begin{subfigure}{.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth, trim=0.01cm 0.01cm 0.01cm 0.01cm, clip=true]{plots/access_mode_rps_barplot.pdf}
    \vspace{-6mm}
    \caption{Throughput in requests/second.}
    \label{fig:ThroughputDiffModes}
    % \vspace{-4mm}
\end{subfigure}
\begin{subfigure}{.5\columnwidth}
	\centering
	\includegraphics[width=\linewidth, trim=0.01cm 0.01cm 0.01cm 0.01cm, clip=true]{plots/boxplot_configuration.pdf}
    \vspace{-6mm}
    \caption{Latency in ms.}
    \label{fig:LatencyDiffModes}
\end{subfigure}
\vspace{-4mm}
\caption{Throughput and latency for different methods of exporting the services for different serverless platforms.}
\label{fig:DiffModes}
\end{figure}

\begin{figure}[htb!]
\begin{subfigure}{.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth, trim=0.01cm 0.01cm 0.01cm 0.01cm, clip=true]{plots/http_payload_rps_barplot.pdf}
    \vspace{-5mm}
    \caption{Throughput in requests/second.}
    \label{fig:ThroughputPayload}
    % \vspace{-4mm}
\end{subfigure}
\begin{subfigure}{.5\columnwidth}
	\centering
	\includegraphics[width=\linewidth, trim=0.01cm 0.01cm 0.01cm 0.01cm, clip=true]{plots/http_payload_latency_cdf.pdf}
    \vspace{-5mm}
    \caption{CDF of Latency.}
    \label{fig:LatencyPayload}
\end{subfigure}
\vspace{-3mm}
\caption{Throughput and latency of different payload sizes for different serverless platforms.}
\label{fig:DiffPayload}
\end{figure}
}

==> Serverless_measurement-12 copy/src/Background.tex <==
%\section{Background}
%Distingusih pulic cloud services vs the self-hosted `FaaS' and scope of our work in the latter. 
%\input{src/ServerlessPlatformDiagrams.tex}

%Table describing the key statistics and features of the 4 serverless platforms.

%\subsection{Types of Serverless platforms}
Several cloud service provides (CSPs) offer serverless computing platforms on their public clouds \eg AWS Lambda functions, Google Cloud Platform, Microsoft Azure, and IBM Bluemix \etc These cloud platforms also offer other supporting services such as an event notification service, storage service, database services \etc that are necessary for operating an overall serverless ecosystem. %to deploy, trigger and execute the serverless functions. 
%Currently these forms of public cloud serverless dominate the serverless market share~\cite{newstack_guide_to_serverless_18}, as they take-away the hassle of building the necessary infrastructure. However, one may argue that these public hosted serverless platforms on the contrary incur greater development and deployment risks due to cloud vendor `lock-in' in terms of the necessary infrastructure support. In addition, they require to architect, design and deploy the serverless functions in a way that bind the usage of the supporting services offered by the cloud. This not only makes the solutions specific to cloud service provider, but also make it difficult to mix-and-match different services, and as well to migrate the functions to either self-hosted servers or to other cloud service provider. 
%Further, a
These CSPs govern many of the function-related characteristics such as: how long functions can run, how long can they be kept %the functions 
idle, the number of concurrent active instances, load balancing among the active instances, retry in the case of failed requests \etc These are
%This leaves for almost no flexibility for the user and be 
almost entirely dependent on the cloud providers' terms and conditions. To understand the impact of these choices, it is useful to study the functioning of
%The other alternative is to leverage the
open source serverless platforms such as Knative, Kubeless, Nuclio, OpenFaaS, OpenWhisk\footnote{\url{https://openwhisk.apache.org}}, \etc

\vspace{-1mm}\subsection{Open-source Serverless platforms}\vspace{-1mm}
Several open source serverless platforms allow us to freely leverage and mix-and-match different open source services, and to deploy and manage the functions on self-hosted clouds. However, the challenges are the i) readiness (requires learning and setup expertise) of the necessary infrastructure and integration of different services, ii) challenges with management and maintenance of the necessary service infrastructure. iii) lack of technical support. 
Hence, in this work we specifically select four of the Kubernetes~\cite{burns2016borg} based open source serverless frameworks based on the recent popularity,\footnote{Until the release of Knative and Nuclio, the Kubeless and OpenFaaS were shown to be the top two leading serverless platforms in terms of current and planned usage~\cite{newstack_serverless_survey_18}} community support and feature richness of these platforms.
\Scut{We illustrate the dependency on Kubernetes - an open-source container orchestration system that automates application deployment, management and scaling. 
We also describe the salient features of these open source serverless platforms.}
%
% \hide{
% First, we briefly describe the 4 major Kubernetes-based open source serverless platforms and their distinct characteristics. We specifically select these four based on the recent popularity,\footnote{Until the release of Knative and Nuclio, the Kubeless and OpenFaaS were shown to be the top two leading serverless platforms in terms of current and planned usage~\cite{newstack_serverless_survey_18}} community support and feature richness of these platforms.

% \subsection{Nuclio}
% Nuclio is both an open source and managed serverless platform powered by Iguazio Systems.\footnote{The open source version that we use does not support the auto-scaling feature} It is considered a high performance serverless platform which can automate the development, operation, and scaling of serverless functions. It can be run with either docker or Kubernetes. 
% The distinct features of Nuclio is the `Processor' architecture which provides work parallelism through multiple worker processes per container. It also supports stateful and data intensive workloads, including support for GPU, and state check-pointing. 
% %It supports code written in different languages (currently supports 8 languages) and currently 14 native triggers/streaming protocols including HTTP, Cron, batch, Kafka, Kinesis, Google pub-sub, Azure event-hub, MQTT, etc. are supported out of the box, and additional triggers can be added dynamically. 
% Nuclio is primarily focused on data analytics and ML workloads.

% \subsection{OpenFaaS}
% OpenFaaS is another framework for building serverless functions, which builds upon industry-standard Cloud Native technology enabling serverless functions with Docker and Kubernetes.  
% The main components of OpenFaaS are the following: i) API gateway and ii) Function watchdog. 
% API gateway provides access (external route) to the functions, collects metrics and provides scaling by interacting with the corresponding orchestration engine (Kubernetes).
% Function watchdog is a tiny Golang HTTP server that serves as the entry point to the container for the HTTP requests to be forwarded to the serverless function. 
% %It provides an unmanaged and generic interface between the outside world and the serverless function. 
% Watchdog marshals the HTTP requests from the API Gateway to invoke the serverless function. It acts as init function and forks the process (function) and passes in the HTTP request via stdin and reads a HTTP response via stdout.
% %A command line interface is used to package each function into a Docker container. 
% Additionally, OpenFaaS provides the AlertManager component (combined with Prometheus) or the Kubernetes Horizontal Pod Autoscaler (HPA) to enable the zero-scale and rate based auto-scaling features.
% The key difference with the OpenFaaS is that any process can become a serverless function through the watchdog component and a Docker container. This allows to run the function coded in any language without any time/duration constraints. 

% \subsection{Knative}
% The Knative builds on top of Kubernetes~\cite{burns2016borg} %and Istio\~cite{istio}, 
% to provide container based runtime for deploying the serverless applications. %with advanced network routing.
% Knative provides a set of building blocks for serverless functions that can be run on top of Kubernetes. It has three main components namely i) Build, ii) Serving and iii) Eventing. 
% The Build component is implemented using a Kubernetes CRD and is a pluggable model for building applications (in containers) from source code. 
% Serving component extends Kubernetes to provide runtime computing support for deploying and running serverless workloads. This component also provides scale-to-zero support based on the received requests, and 
% The Eventing component provides the necessary primitives for consuming and producing events.
% it uses Istio as ingress controller to export the services and for network routing.

% \subsection{Kubeless}
% Kubeless is another Kubernetes based serverless framework, based on the three basic primitives: functions, triggers and runtime. 
% A function is a representation of the code to be executed, and trigger is an event source. 
% A trigger can be associated to a single function or to a group of functions depending on the event source type. A runtime represents a language and runtime specific environment in which a function will be executed.
% The main component of this platform is a CRD controller that continuously watches for changes to function objects and takes the necessary actions, such as creation or deletion of a new function object. The runtime image used to deploy a function can be explicitly specified by the user, the image artifact is generate on-the-fly, or a pre-built image is used where using Kubernetes’ configmap the function code is deployed into the corresponding Kubernetes pod. Upon deletion, the controller releases the used computing resources. %Figure~\ref{fig:kubeless_arch} describes the key components and the working model of serverless functions in Kubeless. Kubeless ensures that the associated function(s) are invoked at least once. 

% }
% \hide{
% https://thenewstack.io/whats-next-serverless/
% However, serverless platforms have challenges which limit their usability and applicability:
% Slow performance and lack of concurrency (single threaded)

% Lock-in to platform specific event and data sources

% Complexity of application state maintenance, code dependencies and service dependencies

% They are impossible to develop, debug, test and deploy in a hybrid or multicloud environment

% Latency of tens or hundreds of milliseconds is the norm today when developing serverless functions in the cloud, and we’re lucky if we manage to run more than a few thousands of events/sec without taking on a second mortgage. This limits the usage to non-performance-sensitive front-end apps or glue logic. Serverless can address many more workloads if it were faster or more efficient.

% https://blog.alexellis.io/introducing-functions-as-a-service/

% 3. Asynchronous processing
% One of the traits of a serverless function is that it's small and fast, typically completing synchronously within a few seconds. There are several reasons why you may want to process your function asynchronously:

% it's an event and the caller doesn't need a result
% it takes a long time to execute or initialize - i.e. TensorFlow / Machine Learning
% you're ingesting a large amount of requests as a batch job
% you want to apply rate limiting
% I started a prototype for asynchronous processing via a distributed queue. The implementation uses the NATS Streaming project but could be extended to use Kafka or any other abstraction that looks like a queue.
% }

==> Serverless_measurement-12 copy/src/Conclusion.tex <==
Through measurements, we explored different open-source %Kubernetes-based 
serverless platforms and identified the key design considerations and their impact on performance and auto-scaling. We show that the interaction between the API Gateway/Ingress controller and the function pods, the overheads of this component and the way requests are queued influence baseline performance. %artifacts of queueing the requests. 
Further, the `RPS'-based and `Concurrency'-based auto-scaling approaches by themselves are insufficient and need to evolve to properly meet workload demands, so that we can avoid maintaining a large number of instances active. %to truly meet the serverless characteristics -- virtually performance of one worker per request, without the overheads of keeping the 
%are still nascent or have matured a lot, but yet to be tuned to meet the serverless characteristics.?
%The opensource serverless frameworks are no more nascent, but gradually maturing and yet present a lot of potential to evolve towards making serverless the pinnacle of cloud. 

==> Serverless_measurement-12 copy/src/Discussion.tex <==
Some of the aspects surrounding the open-source serverless platforms that need additional community attention. 
\begin{itemize}
    \item 
    \item Flexibility vs learning time:
    \item Reliance on Kubernetes services and auto-scaling: Pros and cons
    \item Need for 'rate-cost' proportional scheduling and scaling of services.
    \item Debug and Support service for open-source platforms:
\end{itemize}

==> Serverless_measurement-12 copy/src/Evaluation.tex <==
The main focus of our evaluation is to distinguish and illustrate the impact of the serverless platform specific design choices and their dependency on the Kubernetes orchestration and management services. A second important focus is to understand the auto-scaling capabilities, and the need to go beyond the resource utilization based scaling services provided by Kubernetes. %demonstrate the need of rate-based auto-scaling for serverless platforms beyond 

\vspace{-1mm}\subsection{Experimental setup and Workload description}\vspace{-1mm}
%  and Docker (v18.09.2)
We evaluate the serverless platforms on the Cloudlab testbed~\cite{cloudlab} consisting of one master and two worker nodes, each of them equipped with Intel CPU E5-2640v4@2.4GHz (10 physical cores), running Ubuntu 16.04.1 LTS (kernel 4.4.0-154-generic).
We built all four serverless platforms on Kubernetes (v1.15.3), using the latest version available at the time of writing.\footnote{Nuclio (v1.1.16). OpenFaaS consists of: Gateway (v0.17.0), Faas-netes (v0.8.6), Prometheus (v2.11.0), Alert manager (v0.18.0), Queue worker (v0.8.0) and Faas-cli (v0.9.2), and the HTTP mode of-watchdog. %(which will be the default mode in the future. \knote{whose future?? yours or OpenFaaS??}) 
We use Knative (v0.8) with Istio (v1.1.7) ingress controller, and Kubeless (v1.0.4) with Traefik ingress controller (v1.7).}
% (Python 3.6 runtime is supported by all the serverless platforms)  to implement the serverless functions 
We choose Python 3.6 and implement different serverless functions viz. i) simple Hello-world function as the %most simple 
baseline, and ii) HTTP server function that fetches and serves pages of different sizes from the local HTTP server.
We use %a standard HTTP workload, and use the
\texttt{wrk}~\cite{wrk} %and \texttt{hey}~\cite{hey} 
to generate the HTTP workloads and invoke the serverless functions. \Scut{We detail the platform and workload specific configurations in each of the experiments.} 
%  and \texttt{Apache bench}~\cite{benchab} tools 

\vspace{-1mm}\subsection{Performance - Throughput and Latency}
\vspace{-1mm}\subsubsection{Baseline Performance}~\label{sec:basline_eval}
To evaluate the baseline performance \ie throughput (average requests processed per seconds) and response latency of different serverless platforms, we use a simple `Hello-world' - a no operation function, that  returns 4 bytes of static text in the response. %null response. 
For a fair comparison, we limit to %limited each platform to 
a single instance of the function pod, disable auto-scaling and configured the same queue size and timeout parameters (50K requests, and 10s timeout) at the ingress/gateway and function pod components across all the platforms. For Nuclio, we further restricted it to a single worker process.

\begin{figure}[htb!]\vspace{-0mm}
\begin{subfigure}{0.5\columnwidth}\vspace{-3mm}
    \centering
    \includegraphics[width=\linewidth, trim=0.01cm 0.01cm 0.01cm 0.01cm, clip=true]{plots/hello_barplot_conc_rps-crop.pdf}
    \vspace{-5mm}
    \caption{Avg. throughput.}\Scut{ at different concurrency levels.}
    \label{fig:nullthrput}
\end{subfigure}%
\begin{subfigure}{0.5\columnwidth}\vspace{-3mm}
	\centering
	\vspace{1mm}
    \includegraphics[width=\linewidth]{plots/hello_latency_cdf-crop.pdf}
    \vspace{-5mm}
    \caption{\Scut{CDF of l}Latency for concurrency of 100.}
    \label{fig:nulllatency}
\end{subfigure}%
\vspace{-4mm}
\caption{Throughput and latency of `hello-world' function. % across different serverless platforms. %\knote{Order this as Nuclio, OpenFaaS, Knative and Kubeless. In that order.}
}\label{fig:NULLThroughput}
\vspace{-4mm}
\end{figure}

Fig. \ref{fig:nullthrput} shows the baseline throughput achieved by different platforms for different concurrent executions of requests. Nuclio outperforms the other platforms due to the low overhead of a direct function call. Routing through the API gateway/Ingress controller components incurs not just the overhead for HTTP connection termination, but also for the context-switch/transfer of the packets across the kernel and user-space of the worker node twice to get it routed to the function pod as shown in the Fig.~\ref{fig:svc_export_flannel_arch}. 
To quantify the overhead, we also experimented with Nuclio using an ingress controller mode and observed the overhead. It resulted in almost half the throughput ($\sim$1700 RPS as opposed to $\sim$3000 RPS for direct call) and nearly $2\times$ latency overhead (increases from 356$\mu$s to 611$\mu$s). %its pre-fork worker process model, which persists and multiplexes the processing of requests across functions and 
At the other extreme, Kubeless forks the function for every request, resulting in severely degraded throughput and latency.

From Fig.~\ref{fig:nulllatency}, we can observe that median latency is lowest for Kubeless, and is marginally higher (20$\sim$50 ms) for the queue based frameworks. However, tail latency (above 95\%ile) degrades severely for Kubeless %(due to the dropped requests??) 
and OpenFaaS, while Nuclio and Knative do not see this increased heavy tail-latency. \knote{this sentence is not understandable. Also, call out the two latency graphs as (b) and (c), explain why you have them and then discuss the latency. What you are implying is that the tail latency for Knative is high, right? What do you mean by queue-based? Do you mean concurrency level is 1000?}\sknote{ we wanted to show latency with concurrency=1 (no queuing) and concurrency=1000 (queuing effect) differences, but due to space limits, and small plots, we settled to show only for concurrency=100.} 
%In order to avoid the added queuing latency, we limit the number of maximum in-flight requests to 1 \knote{do you mean concurrency level?? Or are you referring to another parameter, in-flight, that you have not described so far??} for these experiments. 
The results indicate that having process based communication within a container (\eg Nuclio) along with a local worker queue %and associated timeout 
achieves better throughput by having lower overhead for processing requests.
%\noindent\textbf{Takeway}: It is good to have process based communication within a pod (Nuclio) with local worker queue and timeouts for the queued tasks. 

% \input{plots/eval1_plots.tex}

\vspace{-1mm}\subsubsection{HTTP Workload}\label{sec:httpworkload}\vspace{-1mm}
Next, we change to having http-workload.%, where  %%evaluate the throughput of serverless platforms.
%For these experiments, we implement custom python based serverless functions
%%In this experiment, 
%we implement a simple python function that communicates with a local HTTP server (located on Kubernetes master node), %\knote{not understandable},
%and responds with a 4 byte payload for each of the requests. 
%\knote{how is this different than the Hello-World?? Seems equally simple}. \sknote{ Function additionally invokes a HTTP get call on the server running on a master node.} 
Again, we keep the serverless platform settings the same as described in the baseline experiment \S\ref{sec:basline_eval}.
Fig.~\ref{fig:HTTPWorkload} shows the throughput for varying number of concurrent connections and the latency profile for concurrency level of 100. %s for concurrency levels of 1 and 1000 connections.%single concurrent use and 1000 concurrent connections respectively.
Nuclio has the least 99\%ile latency within 500ms,
%Nuclio has the least latency for a concurrency level of 1, since there is no queuing. The latency (even 99\%ile) is within 5ms, except for Kubeless. However, the latency increases drastically to 100$\sim$1000 ms for concurrency level of 1000.
as it allows queuing only within the function pod, while OpenFaaS and Knative can queue requests at ingress/gateway components. OpenFaaS shows heavy tail due to queuing at both the gateway and watchdog components, each having distinct timeout parameters.
Kubeless drops the connections at the ingress, resulting in additional retries from the client - hence it's lower throughput (the lower latency with Kubeless is because it is measured only for those requests that succeed at a concurrency level of 100).
\begin{figure}[htpb!]\vspace{-3mm}
\begin{subfigure}{0.5\columnwidth}\vspace{-0mm}
    \centering
    \includegraphics[width=\linewidth, trim=0.01cm 0.01cm 0.01cm 0.01cm, clip=true]{plots/http_barplot_conc_rps-crop.pdf}
    \vspace{-5mm}
    \caption{Avg. throughput.}\Scut{for different concurrency levels.}
    \label{fig:HTTPRPS}
\end{subfigure}%
\begin{subfigure}{0.5\columnwidth}\vspace{-0mm}
	\centering %width=3.2in
	\vspace{1mm}
	\includegraphics[width=\linewidth, trim=0.01cm 0.01cm 0.01cm 0.01cm, clip=true]{plots/http_latency_cdf-crop.pdf}
    \vspace{-5mm}
    \caption{Latency for concurrency of 100.}
    \label{fig:HTTPCDFLatency}
\end{subfigure}%
\vspace{-4mm}
\caption{Throughput \& latency of `http-workload' function across different serverless platforms at different concurrency levels.} 
% \knote{which is which here??? all the legends have been removed!!}
\label{fig:HTTPWorkload}
\vspace{-4mm}
\end{figure}


\vspace{-2mm}\subsubsection{Variable Payload Size}\vspace{-1mm}
For this experiment, in order to assess the data transfer overhead of serverless platforms, we scale the size of payload in the HTTP response and analyze the overheads and impact of assembling, packaging and transporting the HTTP response payload across different serverless platforms.
In Fig.~\ref{fig:DiffPayload}, we observe that Nuclio performs better for small payload sizes (\ie less than 1KB), while OpenFaaS and Knative perform better for large payloads.
\knote{Need to explain why?? Yes, indeed! Please at least speculate}
\knote{additionally, I do not see any insights up to here based on any of the Wireshark trace analysis you folks did. Is there anything you can say with regard to what you learned from the Wireshark trace analysis??}
\begin{figure}[htpb!]\vspace{-3mm}
\begin{subfigure}{0.5\columnwidth}\vspace{-0mm}
    \centering
    \includegraphics[width=\linewidth, trim=0.01cm 0.01cm 0.01cm 0.01cm, clip=true]{plots/http_payload_rps-crop.pdf}
    \vspace{-5mm}
    \caption{Throughput in requests/second.}
    % \knote{there is something wrong with the x-axis. Why is it in KB???}
    \label{fig:ThroughputPayload}
    % \vspace{-4mm}
\end{subfigure}%
\begin{subfigure}{0.5\columnwidth}\vspace{-0mm}
	\centering
	\vspace{1mm}
	\includegraphics[width=\linewidth, trim=0.01cm 0.01cm 0.01cm 0.01cm, clip=true]{plots/http_payload_latency_cdf-crop.pdf}
    \vspace{-5mm}
    \caption{Latency for 1KB payload.}
    \label{fig:LatencyPayload}
\end{subfigure}%
\vspace{-3mm}
\caption{Throughput \& latency of `http-workload' function with different payload sizes for different serverless platforms.}
\label{fig:DiffPayload}
\vspace{-4mm}
\end{figure}
\vspace{-2mm}


\subsubsection{Impact of different modes of exporting services}\vspace{-1mm}
In order to avoid the added queuing latency, we run the http workload with \texttt{wrk} tool and limit the number of maximum concurrent (in-flight) requests to 1 and repeat the experiment 1000 times. 
Fig.~\ref{fig:es:DiffModes} shows the impact on throughput and latency for three different modes of exporting and invoking the serverless functions. 
\textbf{LC} refers to local call, where the client and function pods reside on the same node in the Kubernetes cluster, and client invokes the function directly using the IP-address of the function pod. Nuclio has marginally better throughput and lower latency than Knative and OpenFaaS, while Kubeless suffers in both latency and throughput. 
\textbf{IG/GW} refers to exporting and invocation of serverless function through the ingress/API gateway components. This mode brings down the throughput across all platforms, and also incurs ($\sim$ 1ms) additional latency than `LC' mode.
\textbf{DC} (direct call) approach is only supported by Nuclio, which exports the function pod using the nodeport service of Kubernetes. DC %has the lowest latency, as it 
avoids the additional routing overheads in the worker node (netfilter rules that translate the packet destination, and forward the packets to the function pod). %However, the throughput is lower than LC approach, due to the additional processing involved in UDP encapsulation that is required to route traffic across the two kubernetes nodes.
\begin{figure}[htpb!]
\begin{subfigure}{0.5\columnwidth}\vspace{-3mm}
    \centering
    \includegraphics[width=\linewidth, trim=0.01cm 0.01cm 0.01cm 0.01cm, clip=true]{plots/access_mode_rps_barplot-crop.pdf}
    \vspace{-6mm}
    \caption{Throughput in requests/second.}
    \label{fig:es:ThroughputDiffModes}
    % \vspace{-4mm}
\end{subfigure}%
\begin{subfigure}{0.5\columnwidth}\vspace{-3mm}
	\centering
	\vspace{1mm}
	\includegraphics[width=\linewidth, trim=0.01cm 0.01cm 0.01cm 0.01cm, clip=true]{plots/access_mode_latency_group_boxplot-crop.pdf}
    \vspace{-6mm}
    \caption{Latency in ms.}
    \label{fig:es:LatencyDiffModes}
\end{subfigure}%
\vspace{-4mm}
\caption{Throughput \& latency for different methods of exporting the services on different serverless platforms.}
\label{fig:es:DiffModes}
\vspace{-4mm}
\end{figure}

\vspace{-1mm}\subsubsection{Analysing the latency impact of serverless platforms}\vspace{-1mm} %breakdown within the function pod
%According to Fig.~\ref{fig:es:DiffModes}, the overhead of ingress/gateway is negligible, but the overhead gap of function pod leads to the performance gap among serverless platforms. In addition, the latency from ingress/gateway to function pod also depends on whether the ingress/gateway and function pod reside in the same worker node. Thus, 
We analyze the delay overheads incurred in processing the serverless functions for different platforms. We breakdown the processing delays within the function pod. For this experiment, we use \texttt{curl} to send one request for `hello-world' function and use \texttt{tcpdump} to capture the packets on the worker node of the function pod. We record four timestamps,
%We get four timestamps from \texttt{tcpdump} files, 
\ie (1) when the request reaches the function pod; (2) start of the function runtime; (3) end of the function runtime; (4) when the response is sent out of function pod.  
Time intervals between these timestamps are shown in Fig.~\ref{fig:LatencyBD}.
In all frameworks, the actual run-time of the function (0.001ms) is the same. However, the function initiation time (time taken for request to be forwarded to the function instance) and function response delay (time taken for the response of the function to be sent out of the pod) vary. This depends on how the data is packaged and shared with the function instance. Also, Kubeless (due to forking per request), incurs very high delay in forwarding the packet to the function instance. We also experimented with the 'http-function' and found the startup and response delay overheads to be same.
% \begin{table}[!htbp]
% \vspace{-3mm}
% \centering
% \caption{Latency breakdown of `hello-world' function across different serverless platforms (in ms).}
% \vspace{-3mm}
% \begin{tabular}{c|ccc}
% \hline
% Process & 1\rightarrow2 & 2\rightarrow3 & 3\rightarrow4 \\
% \hline
% Nuclio & 0.63 & 2.84 & 0.54 \\
% OpenFaaS & 1.32 & 2.70 & 0.93 \\
% Knative & 1.30 & 5.30 & 0.62 \\
% Kubeless & 4.96 & 9.65 & 2.63 \\
% \hline
% \end{tabular}
% \label{table:LatencyBD}
% \vspace{-4mm}
% \end{table}

\begin{figure}[!htb]\vspace{-3mm}
    \centering
    \begin{minipage}{0.34\columnwidth}
    \vspace{0pt}
        \centering
        \includegraphics[width=0.7\linewidth, trim=0.01cm 0.01cm 0.01cm 0.01cm, clip=true]{plots/latency_breakdown.pdf}
        \vspace{-1mm}
        % \caption{Diagram of four timestamps}
        \label{fig:LatencyBD-1}
    \end{minipage}
    \begin{minipage}{.65\columnwidth}
    %\resizebox{0.5\linewidth}{!}{
        \centering
        \captionsetup{type=table} %% tell latex to change to table
        \vspace{0pt}
        \begin{tabular}{c|ccc}
        \hline
        Process & 1$\rightarrow$2 & 2$\rightarrow$3 & 3$\rightarrow$4 \\
        \hline
        Nuclio & 0.63 & 0.001 & 0.54 \\
        OpenFaaS & 1.32 & 0.001 & 0.93 \\
        Knative & 1.30 & 0.001 & 0.62 \\
        Kubeless & 4.96 & 0.001 & 2.63 \\
        \hline
        \end{tabular}
        \vspace{-1mm}
        % \caption{Latency breakdown in ms.}
        \label{table:LatencyBD-2}
        %}
    \end{minipage}
    \vspace{-3mm}
    \caption{Latency breakdown (ms) parts of serverless execution.}
    \label{fig:LatencyBD}
    \vspace{-4mm}
\end{figure}

% RAW data got from wireshark/tcpdump:
% Nuclio: 526.414, 527.046, 529.881, 530.426
% OpenFaaS: 627.616, 628.937, 631.637, 632.566
% knative: 258318.211, 258319.515, 258324.811, 258325.433
% Kubeless: 885.225, 890.182, 899.829, 902.456

\vspace{-1mm}\subsection{Auto-scaling}\label{eval:autoscaling}\vspace{-1mm}
Auto-scaling capabilities exported by different serverless platforms vary. Here, we compare the auto-scaling features of Knative and OpenFaaS for both the rate-based and Kubernetes-based horizontal-pod-autoscaler (HPA) modes under different workload characteristics. 
For a fair comparison, we tune the auto-scaling related configuration parameters in both the platforms to have the same interval for the auto-scale triggers and factors for scaling functions.\footnote{In Knative, we disable panic mode, and set the minScale and maxScale instances as 1 and 10, target to 10, max-scale-up-rate to 100, tick interval to 2s, and stable window to 10s, which ensures triggering auto-scale notifications on a 2s window and scaling to 1 or more instances at a time. Likewise, for OpenFaaS, we set scale-factor to 10 and configure the alert-notification window to 2s, and RPS threshold to 10. For HPA, we set CPU limits to 50.} We use the same python function as in \S\ref{sec:httpworkload}.
\noindent\textbf{Note:} In OpenFaaS, auto-scaling is based on the average rate of the incoming requests %observed for a function type 
% (offered load); %irrespective of the rps observed on individual instances, 
(RPS);
in Knative, auto-scaling is based on the concurrency level observed per function instance. The subtle difference is that the average RPS value can be lower or higher than the observed concurrency depending on whether the time for processing a function invocation is higher or lower respectively. We will demonstrate the benefit and deficiency of both approaches. \hide{say autoscale_threshold qps=10, c=10 for scaling, case 1: if workload has rps=11 unbounded traffic, OF will scale, KN=?
case 2: processing cost = 1ms then OF and KN will both scale while 
case 3: processing cost = 1sec
case 4: 
}
\vspace{-1mm}\subsubsection{Workload based auto-scaling}\vspace{-1mm}
%\subsubsubsection{Steady workload}\label{eval:steadyhttp}
\textbf{Steady workload}:
%For this case, 
We use the \texttt{wrk} tool, set a steady rate for outstanding requests (concurrency of 100) and run the experiment for 60s.
%\knote{the workload is fixed throughout the entire period, right? To have a steady outstanding number of requests at 100? Say this a bit more directly.}\sknote{okay}
Also, to enforce proper traffic distribution across newly created pods, we force the OpenFaaS gateway to terminate and reestablish connections with the function pods.
Periodically, every 2s, we monitor the number of pod instances, CPU and memory usage, and throughput.
From Fig.~\ref{fig:Autoscaling-qps-steady}, we observe that Knative scales multiple instances at a time to reach the max. (10) instances quickly (in 12s), %and provides higher average throughput, 
while OpenFaaS just scales up one instance at a time, taking 26s to scale up to the max. (10) instances. 
% We omit the steady state results  in the plots. 
Although, the CPU usage for the scaled instances looks identical, the memory pressure is higher for Knative. This stems from the difference in the python runtimes and overheads in the queue-proxy container component for Knative and of-watchdog components in OpenFaaS.
  
\begin{figure}[htb!]
\begin{subfigure}{0.5\columnwidth}\vspace{-3mm}
    \centering
    \includegraphics[width=\linewidth, trim=0.01cm 0.01cm 0.01cm 0.01cm, clip=true]{plots/autoscale_rps_cpu_memory_knative_steady_20190913_191941_10_stable_win-crop.pdf}
    \vspace{-5mm}
    \caption{Knative.}
    \label{fig:Autoscaling-qps-steady-knative}
    % \vspace{-4mm}
\end{subfigure}%
\begin{subfigure}{0.5\columnwidth}\vspace{-3mm}
	\centering
	\includegraphics[width=\linewidth, trim=0.01cm 0.01cm 0.01cm 0.01cm, clip=true]{plots/autoscale_rps_cpu_memory_openfaas_steady_20190913_203342-crop.pdf}
    \vspace{-5mm}
    \caption{OpenFaaS.}
    \label{fig:Autoscaling-qps-steady-openfaas}
\end{subfigure}%
\vspace{-3mm}
\caption{Auto-scaling with steady workload.}% for different serverless platforms.}
\label{fig:Autoscaling-qps-steady}
\end{figure}
\vspace{-4mm}

% \begin{figure}[htb!]
% \begin{subfigure}{0.5\columnwidth}
%     \centering
%     \includegraphics[width=\linewidth, trim=0.01cm 0.01cm 0.01cm 0.01cm, clip=true]{plots/autoscale_rps_cpu_memory_knative_steady_20190913_191941_10_stable_win}
%     \vspace{-5mm}
%     % \caption{Knative.}
%     \label{fig:Autoscaling-fct-1}
%     % \vspace{-4mm}
% \end{subfigure}
% \vspace{-3mm}
% \caption{FCT and max number of pods of QPS-based auto-scaling on fix number of requests for different serverless platforms.}
% \label{fig:Autoscaling-fct}
% \end{figure}

% Note for issue figure: Knative: continuous traffic sent by wrk, 9 concurrent requests; OpenFaaS: continuous traffic sent by wrk, 9 concurrent requests.


%\subsubsection{Bursty workload}
\noindent \textbf{Bursty workload}
We also experimented by varying the http workload to have bursts of concurrent requests %by sending large number of concurrent requests 
followed by a large idle period. Fig.~\ref{fig:Autoscaling-qps-bursty} shows that, Knative is more responsive to bursts, and is able to scale quickly to a large number of instances, %resulting in performance improvement. However, 
while OpenFaaS scales %more 
gradually %. OpenFaaS 
and has lower average throughput.

% In one period, we use \texttt{wrk} to send traffic for 30s with 100 concurrent requests and sleep for 60s. We show 2 periods.
%We should at least do one experiment with bursty workload if possible.

\begin{figure}[htb!]
\begin{subfigure}{0.5\columnwidth}\vspace{-3mm}
    \centering
    \includegraphics[width=\linewidth, trim=0.01cm 0.01cm 0.01cm 0.01cm, clip=true]{plots/autoscale_rps_cpu_memory_knative_bursty_20190914_042105-crop.pdf}
    \vspace{-5mm}
    \caption{Knative.}
    \label{fig:Autoscaling-qps-bursty-knative}
    % \vspace{-4mm}
\end{subfigure}%
\begin{subfigure}{0.5\columnwidth}\vspace{-3mm}
	\centering
	\includegraphics[width=\linewidth, trim=0.01cm 0.01cm 0.01cm 0.01cm, clip=true]{plots/autoscale_rps_cpu_memory_openfaas_bursty_20190914_045001-crop.pdf}
    \vspace{-5mm}
    \caption{OpenFaaS.}
    \label{fig:Autoscaling-qps-bursty-openfaas}
\end{subfigure}%
\vspace{-3mm}
\caption{Auto-scaling with bursty workload.}% for different serverless platforms.}
\label{fig:Autoscaling-qps-bursty}
\end{figure}
\vspace{-4mm}

%\noindent\textbf{Uniformly increasing workload}
% \subsubsection{Uniformly increasing workload}

% \begin{figure}[htb!]
% \begin{subfigure}{0.5\columnwidth}
%     \centering
%     \includegraphics[width=\linewidth, trim=0.01cm 0.01cm 0.01cm 0.01cm, clip=true]{plots/autoscale_rps_cpu_memory_knative_steady_20190913_191941_10_stable_win}
%     \vspace{-5mm}
%     \caption{Knative.}
%     \label{fig:Autoscaling-qps-inc-knative}
%     % \vspace{-4mm}
% \end{subfigure}
% \begin{subfigure}{0.5\columnwidth}
% 	\centering
% % 	\includegraphics[width=\linewidth, trim=0.01cm 0.01cm 0.01cm 0.01cm, clip=true]{plots/autoscale_rps_cpu_memory_knative_steady_20190913_191941_10_stable_win}
%     \vspace{-5mm}
%     \caption{OpenFaaS.}
%     \label{fig:Autoscaling-qps-inc-openfaas}
% \end{subfigure}
% \vspace{-3mm}
% \caption{Throughput and metrics of QPS-based auto-scaling on uniformly increasing workload for different serverless platforms.}
% \label{fig:Autoscaling-qps-inc}
% \end{figure}

% \begin{figure}[htb!]
% \begin{subfigure}{0.5\columnwidth}
%     \centering
%     \includegraphics[width=\linewidth, trim=0.01cm 0.01cm 0.01cm 0.01cm, clip=true]{plots/autoscale_rps_cpu_memory_knative_steady_20190913_191941_10_stable_win}
%     \vspace{-5mm}
%     \caption{Knative.}
%     \label{fig:Autoscaling-hpa-inc-knative}
%     % \vspace{-4mm}
% \end{subfigure}
% \begin{subfigure}{0.5\columnwidth}
% 	\centering
% % 	\includegraphics[width=\linewidth, trim=0.01cm 0.01cm 0.01cm 0.01cm, clip=true]{plots/autoscale_rps_cpu_memory_openfaas_20190909_221233}
%     \vspace{-5mm}
%     \caption{OpenFaaS.}
%     \label{fig:Autoscaling-hpa-inc-openfaas}
% \end{subfigure}
% \vspace{-3mm}
% \caption{Throughput and metrics of HPA-based auto-scaling on uniformly increasing workload for different serverless platforms.}
% \label{fig:Autoscaling-hpa-inc}
% \end{figure}

\begin{figure}[htb!]\vspace{-3mm}
\begin{subfigure}{0.5\columnwidth}\vspace{-3mm}
    \centering
    \includegraphics[width=\linewidth, trim=0.01cm 0.01cm 0.01cm 0.01cm, clip=true]{plots/autoscale_rps_cpu_memory_knative_steady_issue_20190914_065536-crop.pdf}
    \vspace{-5mm}
    \caption{Knative.}
    \label{fig:Autoscaling-issue-knative}
    % \vspace{-4mm}
\end{subfigure}%
\begin{subfigure}{0.5\columnwidth}\vspace{-2mm}
	\centering
	\includegraphics[width=\linewidth, trim=0.01cm 0.01cm 0.01cm 0.01cm, clip=true]{plots/autoscale_rps_cpu_memory_openfaas_steady_issue_20190914_060628-crop.pdf}
    \vspace{-5mm}
    \caption{OpenFaaS.}
    \label{fig:Autoscaling-issue-openfaas}
\end{subfigure}%
\vspace{-3mm}
\caption{Auto-scaling issues with Knative and OpenFaaS.}
\label{fig:Autoscaling-issue}
\vspace{-4mm}
\end{figure}

%\subsubsection{Challenges with auto-scaling in OpenFaaS and Knative.}\label{eval:auto:issue}
\noindent\textbf{Issues with auto-scaling in OpenFaaS and Knative}:
%\subsubsection{Rate or Concurrency based auto-scaling?}
%\textbf{concurrency based auto-scaling} 
In another experiment, we use the same setup as in the steady workload %(\S \ref{eval:steadyhttp})
experiment, but lower the number of outstanding requests from 100 to 9. 
From Fig.~\ref{fig:Autoscaling-issue}, we observe that Knative fails to auto-scale and continues to operate with just 1 function pod instance, resulting in almost 7$\times$ lower (200 RPS) throughput compared to the earlier case (1500 RPS).
%To demonstrate the differences and to highlight the observed issues with leveraging Kubernetes for rps based scaling. We 
Next, we revert to vanilla OpenFaaS (\ie as in github, and disable the workaround of resetting the connections to the function pods), and run the same steady workload experiment. The function pods get auto-scaled as before. But, the throughput shows no improvement. Also, note that with auto-scaling the memory usage increases, but CPU utilization remains steady. We found the issue to be due to incorrect traffic distribution. Due to the long running connections (setup by OpenFaaS gateway at the beginning with the first function pod), all the traffic is just routed only to the first function pod, while the remaining, newly scaled pods, do not receive any traffic.\footnote{%We raised this bug with the OpenFaaS community: 
Bug raised: \url{https://github.com/openfaas/faas/issues/1303}.}




\vspace{-3mm}\subsubsection{Resource based auto-scaling}\vspace{-1mm}
We use the same setup (steady state), configure the cpu usage limit to 50\%, and leverage Kubernetes HPA for auto-scaling. Note, the auto-scaling of function pods is governed by Kubernetes only. %, and there are no additional serverless platform specific configurations required. %However, the CPU utilization of the function pod depends on the serverless platform specific components (event-listener, of-watchdog, queue-proxy). 
From Fig.~\ref{fig:Autoscaling-hpa-steady}, we can observe that, except for Kubeless, the auto-scaling behavior is same across all the platforms \ie auto-scaling tries to double the instances at each step until it reaches the maximum (10). However, the duration of each step depends on the CPU utilization factor, which in turn depends on the serverless platform specific components (event-listener, of-watchdog, queue-proxy). Nuclio, being relatively more CPU hungry is able to scale more rapidly (in 40s), than Knative and OpenFaaS. %With Kubeless, we observed that due to fork per request model, not only the throughput, but also the cpu utilization remains low. Hence, it does not scale too many instances (3 instances in 100s). %We observed at most 3 instances being created for Kubeless. 
With Kubeless, the fork-per-request results in high latency, dropping of incoming requests that in turn results in low throughput and low CPU utilization. Thus, it results in poor auto-scaling as well. 


\begin{figure}[htb!]\vspace{-1mm}
\begin{subfigure}{0.5\columnwidth}
    \vspace{-2mm}
    \centering
    \includegraphics[width=\linewidth, trim=0.01cm 0.01cm 0.01cm 0.01cm, clip=true]{plots/autoscale_rps_cpu_memory_nuclio_steady_20190915_164326-crop.pdf}   
    \vspace{-6mm}
    \caption{Nuclio.}
    \label{fig:Autoscaling-hpa-steady-nuclio}
    % \vspace{-4mm}
\end{subfigure}%
\begin{subfigure}{0.5\columnwidth}\vspace{-3mm}
	\centering
	\includegraphics[width=\linewidth, trim=0.01cm 0.01cm 0.01cm 0.01cm, clip=true]{plots/autoscale_rps_cpu_memory_openfaas_hpa_steady_20190915_132123-crop.pdf}
    \vspace{-6mm}
    \caption{OpenFaaS.}
    \label{fig:Autoscaling-hpa-steady-openfaas}
\end{subfigure}
\begin{subfigure}{0.5\columnwidth}\vspace{-1mm}
    \centering
    \includegraphics[width=\linewidth, trim=0.01cm 0.01cm 0.01cm 0.01cm, clip=true]{plots/autoscale_rps_cpu_memory_knative_hpa_steady_20190915_101643-crop.pdf}
    \vspace{-6mm}
    \caption{Knative.}
    \label{fig:Autoscaling-hpa-steady-knative}
    % \vspace{-4mm}
\end{subfigure}%
\begin{subfigure}{0.5\columnwidth}\vspace{-1mm}
    \centering
    \includegraphics[width=\linewidth, trim=0.01cm 0.01cm 0.01cm 0.01cm, clip=true]{plots/autoscale_rps_cpu_memory_kubeless_hpa_steady_20190915_184906-crop.pdf}
    \vspace{-6mm}
    \caption{Kubeless.}
    \label{fig:Autoscaling-hpa-steady-kubeless}
    % \vspace{-4mm}
\end{subfigure}%
\vspace{-4mm}
\caption{HPA-based auto-scaling on steady workload.}% for different serverless platforms.}
\label{fig:Autoscaling-hpa-steady}
\vspace{-6mm}
\end{figure}

% \hide{
% \begin{figure}[htb!]
% \begin{subfigure}{0.5\columnwidth}
%     \centering
%     \includegraphics[width=\linewidth, trim=0.01cm 0.01cm 0.01cm 0.01cm, clip=true]{plots/autoscale_rps_cpu_memory_knative_steady_20190913_191941_10_stable_win}
%     \vspace{-5mm}
%     \caption{Knative.}
%     \label{fig:Autoscaling-hpa-bursty-knative}
%     % \vspace{-4mm}
% \end{subfigure}
% \begin{subfigure}{0.5\columnwidth}
% 	\centering
% % 	\includegraphics[width=\linewidth, trim=0.01cm 0.01cm 0.01cm 0.01cm, clip=true]{plots/autoscale_rps_cpu_memory_openfaas_20190909_221233}
%     \vspace{-5mm}
%     \caption{OpenFaaS.}
%     \label{fig:Autoscaling-hpa-bursty-openfaas}
% \end{subfigure}
% \vspace{-3mm}
% \caption{Metrics of HPA-based auto-scaling on bursty workload for different serverless platforms.}
% \label{fig:Autoscaling-hpa-bursty}
% \end{figure}
% }

% \hide{
% \subsection{Reliability}
% \subsubsection{Worker Node Failure}
% \subsubsection{Infrastructure component Failure}
% }

==> Serverless_measurement-12 copy/src/Introduction.tex <==
%%Para1: Serverless Computing. -- what is it,  its impact. new emerging platforms
%%para2: New emergine platforms, (kubernetes based), 
Serverless computing has ushered in a new era in cloud computing. 
%\blfootnote{$^\star$ Work done while visitng UC Riverside.}
%The fundamental appeal of c
Cloud computing 
%arises from the exploitation of virtually infinite amount of shared resources, which in turn enables 
seeks to provide compute and storage services at large scale and low cost to end-users through economies of scale and effective multiplexing.    
%It's fundamental appeal arises from the exploitation of multiplexing computing and storage by sharing resources and thus lowering costs to end-users. 
Serverless computing takes this multiplexing and scalability to the next level by allowing providers to commit just the required amount resources to a particular application 
%to a minimal level 
(as many instances as necessary, but only when needed) and utilize the resources for just the time needed to execute an invoked function. Resources are scaled dynamically to meet the demand from user requests.
Unlike the `traditional' cloud deployment model%\eg Amazon EC2 (Elastic Compute cloud)
, where the number of necessary compute instances are deployed well in advance,
serverless computing allows the cost to be near zero when there is no demand, and scales to as many instances as needed to meet the traffic demand. Thus, serverless  is meant to be both scalable and more cost effective. 

%Another key aspect of serverless is less-management' 
In addition to scaling and multiplexing, serverless computing allows developers to build, deploy and run the application on demand without focusing on server management, according to the Cloud Native Computing Foundation (CNCF)~\cite{yaroncncf}.  %refers to the concept of building and running applications that do not require server management. This  as  one or more cloud native functions, and the serverless platform to execute the required functions based on the demand.
%In other words, the computing resources that are necessary for function execution are provisioned only when they are needed to be executed. 
When an event is triggered, a piece of infrastructure is allocated dynamically to execute the code. %\footnote{
The underlying details of resource management: resource allocation, communication of user data, and the execution of functions is abstracted from the user.
%} 
%what happens under the covers is a Linux container is started on a machine and details - metadata about the event - is passed into the container at the point of execution.
%Serverless computing can be regarded as an evolution of cloud computing service models from Infrastructure-as-a-Service (IaaS), 
%Platform-as-a-Service (PaaS) to Function-as-a-Service (FaaS). %With IaaS, only the underlying infrastructure (hardware resources) are abstracted out from the user to deploy the virtual resources, while with PaaS abstracts the entire platform (operating system and system software) to build and deploy the applications, the FaaS takes a step further and abstracts the management and deployment of applications including the programming runtime to provide just the necessary options to readily deploy a piece of code and execute without worrying about its deployment.
%To re-check from here %
Serverless computing %provides a new approach to
manages cloud resources typically by deploying applications in dynamically instantiated containers. For instance, Amazon provides AWS-Lambda~\cite{awslambda}, an event-driven, serverless computing platform that enables to implement and deploy application code in any of the supported languages %(Python, NodeJS, Java, C\#, Go, Ruby, and Powershell), 
and execute on-demand as docker-containers. The serverless infrastructure manages the queuing of requests and can automatically scale %backend service 
containers to meet fluctuating demands. 

%The elastic nature of serverless computing makes it an ideal match for edge computing data centers, where the small scale of each site places tight restrictions on the number of servers that can be deployed there. Unlike mega-data-centers, the limited capacity of an edge data center requires efficient use of resources with applications only consuming the resources they need.  This minimizes waste and fragmentation compared to the traditional approach of deploying fixed size virtual machines with dedicated resources for time periods of hours or days.

%Edge computing~\cite{hu2015mobile} seeks to provide more responsive service to users, with the promise of access to shared computing and storage with low latency, thus enabling and encouraging offloading processing from end-devices. It also reduces core bandwidth costs by moving cloud-resident applications closer to users. 
%Reducing the latency costs from tens of milliseconds to one millisecond opens a new range of cloud application types related to Cyber Physical Systems (CPS) and the Internet of Things (IoT)~\cite{hu2015mobile}. Applications such as autonomous vehicle control and live sensor feed analysis require both strong performance and reliability guarantees, \eg mission critical communication IoT use cases such as factory automation and autonomous vehicles demand latency in the range of $250\mu$s-10ms and a reliability of $10^{-9}$ packet loss rate~\cite{schulz2017latency}.

%Unfortunately, the combination of serverless and edge computing is not as perfect a fit as it initially appears.  It is well known that serverless computing can incur high overhead if requests reach a ``cold'' service, causing delays on the order of hundreds of milliseconds to instantiate a new container.  

Our focus is
%In this paper, we focus 
not only on the evaluation and comparison of performance, but seek to identify the key differences in the workings of different Kubernetes-based open-source serverless platforms.
%a second, less explored challenge: the difficulty of providing reliable processing with a serverless-based infrastructure. Just as people have come to depend on network-based services and cloud computing facilities to be as reliable as their own dedicated computing systems, serverless computing needs to evolve and mature to achieve the same reliability expectations. We believe that the limited reliability semantics of today's serverless platforms (\eg AWS Lambda and Microsoft Azure functions support only at-least once semantics) poses high risk for emerging CPS and IoT applications, leaving them truly ``living on the edge'' in terms of the risk of failure and its consequences.
%A number of the edge computing applications mentioned above depend on high throughput and low latency processing of streaming applications. While `traditional' stream processing frameworks are designed for applications with dedicated resources (at least for significant time periods), their functionality is likely to be needed in the serverless context. Moreover, they typically reside on large-scale data centers that are built and managed for being resilient to failures with redundant resources, we see them having to also evolve to be supported on edge data centers.  Furthermore, the edge computing applications such as for IoT and CPS as well as even some vehicular applications may have varying reliability requirements. Some, by the nature of disseminating and processing data in an idempotent manner may require little or no reliability guarantees, and `only' require good responsiveness. On the other hand, there are many applications, such as vehicular safety, processing medical data etc., that require high reliability, and the environment needs to be robust to failures. Thus, it is useful to understand the costs of providing failure resiliency of these stream processing frameworks so that we can examine their utility for serverless computing in an edge computing environment, and also how this failure resiliency can be configured appropriately on an as-needed basis.
%In this paper w
We systematically identify the strengths and deficiencies of 
%the different Kubernetes-based open-source serverless platforms namely the
Knative\footnote{\url{https://github.com/knative}}, Kubeless\footnote{\url{https://kubeless.io}}, Nuclio\footnote{\url{https://nuclio.io}} and OpenFaaS\footnote{\url{https://www.openfaas.com}}. Our key contributions include:
\begin{itemize}
    \item We provide an understanding of the role and interaction of the different components of each of these platforms. 
    \item We describe the impact of key configuration parameters of different components (platform, gateway, controller and function).
    \item We evaluate the mode and operation of auto-scaling supported by these different platforms for different kinds of workloads.% (burst and steady). %and gradually increasing load.) 
%    \item we also evaluate the service reliability guarantees provided by these different platforms.
\end{itemize}
 
%We evaluate the costs associated with providing different reliability guarantees. %during the normal processing. 
%We use Apache-Storm/Trident~\cite{Storm} and Apache-Kafka~\cite{Kafka} stream processing frameworks to evaluate the throughput, latency, and resource cost associated with request processing ranging from best effort service to exactly once guarantees.




==> Serverless_measurement-12 copy/src/Related_Work.tex <==
%We discuss some of the relevant serverless works.
\noindent \textbf{Serverless Platform comparison}: In work~\cite{mcgrath2017serverless, wang2018peeking}, the authors conducted several measurements on different cloud serverless platforms (AWS Lambda, Microsoft Azure, Google Cloud), and found the AWS to be better in terms of throughput, scalability, cold-start latency.  The works~\cite{lloyd2018serverless,cui2} investigate the different factors that influence the performance of AWS lambda, namely the impact of the choice of language of the function, memory footprint of the function, \etc Work~\cite{mohanty2018evaluation} evaluates the performance of Fission, Kubeless and OpenFaaS serverless frameworks and characterizes the response time and the ratio of successfully completed requests for different loads. However the work fails to characterize the throughput of these platforms and accounts for the mean latency (response time) and successful responses at different load characteristics, which is debatable, without the proper consideration and configuration of the serverless platform specific configuration parameters, resulting in inaccurate results. %Further, the work fails to provide key insights on the impact of configuration parameters and provide the insight on 
In the most recent work~\cite{palade}, the authors quantitatively evaluate  Apache OpenWhisk, OpenFaas, Kubeless, and Knative platforms. The results for Kubeless are similar, but for the other platforms, we feel the presented results are inaccurate. This could be due to the usage of Kubernetes. %We observe that performance (throughput) for kubeless to be similar our setup, however the other platforms seem to be 
In contrast, our work focuses on discerning the architectural blocks that impact the performance of Kubernetes based open-source serverless platforms.

==> Serverless_measurement-12 copy/src/ServerlessCompare.tex <==
%We illustrate the dependency on Kubernetes - an open-source container orchestration system that automates application deployment, management and scaling. We also describe the salient features of the open source serverless platforms.  
%Kubernetes is a portable, extensible, open-source platform for managing containerized workloads and services, that facilitates both declarative configuration and automation. It has a large, rapidly growing ecosystem. Kubernetes services, support, and tools are widely available
\vspace{-1mm}\subsection{Dependency on Kubernetes}\vspace{-1mm}
Kubernetes is a portable and extensible platform that facilitates both declarative configuration and automation of deployment and management of containerized workloads. The serverless frameworks rely on Kubernetes APIs for orchestration and management of the serverless functions. \Scut{Figure~\ref{fig:kubernets_svcs} shows the key functions and services of Kubernetes that the serverless frameworks depend on. They}Serverless platforms typically extend and provide the Custom Resource Definition (CRD) features necessary to create and deploy the container pods (group of containers). They depend primarily on Kubernetes for i) Configuration management of containers and pods; ii) Pod scheduling and service discovery; iii) Update roll-outs for functions; and iv) Replication management.% and load-balancing. 



\vspace{-1mm}\subsection{Salient Characteristics of Serverless Platforms}\vspace{-1mm}
Fig.~\ref{fig:serverless_platforms_arch} shows the framework and key components of the 4 different serverless platforms considered in this work.
%we consider in this paper. 
\Scut{We briefly discuss their salient features, their distinct configuration parameters and how their settings influence baseline performance. % for these serverless platforms.
}
%\vspace{-1mm}\subsubsection{Nuclio}\label{ssec:nuclio}\vspace{-1mm}
\\\noindent{\bf Nuclio}:
\Scut{Nuclio is both an open source and managed serverless platform supported by Iguazio Systems.\footnote{The opensource version does not support the auto-scaling feature.} 
%It is considered a high performance serverless platform which can automate the development, operation, and scaling of serverless functions. 
%It can be run along with either Docker or Kubernetes. 
}
Fig.~\ref{fig:nuclio_arch} shows the key components of Nuclio.
The distinct feature of Nuclio is the `Processor' architecture which provides work parallelism through multiple worker processes that can run in each container. 
%It also supports stateful and data intensive workloads, including support for GPU, and state check-pointing. 
%It supports code written in different languages (currently supports 8 languages) and currently 14 native triggers/streaming protocols including HTTP, Cron, batch, Kafka, Kinesis, Google pub-sub, Azure event-hub, MQTT, etc. are supported out of the box, and additional triggers can be added dynamically. 
%Nuclio is primarily focused on data analytics and ML workloads. \knote{why do we need to say this last sentence?} \sknote{Okay, the Nuclio webpage stresses on this aspect as being distinct from other serverless platforms.}
First, the Nuclio service model supports invocation of the `function' pod directly from an external client, without the need for any ingress controller or API gateway. 
Second, the function pod consists of two kinds of processes namely the i) event-listener and ii) one or more worker (user deployed function) processes.
Note, the event-listener can be configured with a timeout parameter to control how long events can be queued\Scut{ there before expiring, while the requests are waiting for processing. Thus, %parameter, implies 
the process can queue multiple requests for processing}. 
%The event-listeners also guarantee exactly-once or at-least-once event execution and handle execution failures.
Third, the number of worker processes can be setup as a static configuration parameter. This enables the function pod to run a desired amount of function instances as different processes, and allows parallel execution on a multi-core node.  % This can result in out-of-order response for the queued events even when the execution of queued events is  guaranteed to be in order.
%Further, the Nuclio supports both `at-least once' and `exactly-once' processing model for the queued events.;  

%\vspace{-3mm}
% (todo: change to helloworld workload)
\begin{figure}[htbp!]\vspace{-2mm}
\begin{subfigure}{.5\columnwidth}
% \begin{subfigure}{.25\textwidth}
    \centering
    \includegraphics[width=\linewidth]{plots/nuclio_worker_perf_rps-crop.pdf}
    \vspace{-6mm}
    \caption{Throughput in requests/second.}
    \label{fig:nuclio_worker_perf}
\end{subfigure}%
\begin{subfigure}{.5\columnwidth}
% \begin{subfigure}{.25\textwidth}
    \centering
    \vspace{1mm}
    \includegraphics[width=\linewidth]{plots/nuclio_worker_perf_cdf-crop.pdf}
    \vspace{-6mm}
    \caption{Latency in ms.}
    \label{fig:nuclio_worker_lat}
\end{subfigure}%
\vspace{-4mm}
\caption{Throughput and latency for different number of workers within one Nuclio function pod (100 concurrent requests).}
\label{fig:nuclio_worker}
\vspace{-5mm}
\end{figure}
To quantify the benefit of having multiple workers, we experimented with simple `http-workload' where  we  implement a  simple  python  function  that  communicates  with  a  local  HTTP server (located on Kubernetes master node), to fetch and respond with a 4 byte payload for each of the requests. %function  with the open source version of Nuclio on the NSF Cloudlab testbed~\cite{cloudlab}. 
Fig.~\ref{fig:nuclio_worker_perf} shows the impact on throughput and latency for multiple workers. We observe a $4\times$ throughput increase with 4 workers and almost $10\times$ improvement with 50 workers. Note, scaling the number of workers also improves the latency as shown in Fig.~\ref{fig:nuclio_worker_lat}. \Scut{Scaling more workers than the physical cores however only marginally improves the throughput. But more importantly, we find that it adversely impacts the tail latency, because of queuing effects.}
\Scut{However, scaling more workers than physical cores adversely impacts the tail latency due to queuing effect.}%has adverse impact on the tail latency due to queuing effect.}%\knote{check the last sentence: it is only the tail latency that is impacted with 50 workers.}  \sknote{yes, it is only the tail latency above 80\%ile that get impacted.} 
% , where each worker node has 20 CPU cores


%\vspace{-1mm}\subsubsection{OpenFaaS}\vspace{-1mm}
\noindent{\bf OpenFaaS}:
% \Scut{OpenFaaS %builds upon industry-standard Cloud Native technology enabling serverless functions with Docker and Kubernetes. It 
% is developed by Alex Ellis, and is currently a registered open-source product of OpenFaaS limited~\cite{alex_openFaas}. %was supported by the Open Source Technology Center (OSTC) at VMware~\cite{alex_openFaas}.
% %\knote{who supports it? What is its distinct feature and does it support stateful functions? I am trying to make sure we describe each of the platforms the same way.}\sknote{yes, will do.}
% The distinct feature of OpenFaaS is the system built-in support for deferred execution %\ie it enables %to process 
% %any OpenFaaS function to be executed synchronously or asynchronously without any adaptations. 
% %In asynchronous mode, 
% where the actual function execution is deferred for later execution, while the client gets an immediate response from the API-gateway based on the queued status of the task. % When a function is called asynchronously the caller gets an instant response and the work is run later on.
% }
The 
%main components of OpenFaaS are: i) API gateway and ii) Function Watchdog. 
%These along with the 
key components of OpenFaaS are shown in Figure~\ref{fig:openfaas_arch}. The API gateway provides access to the functions from outside the Kubernetes cluster (external 
%\knote{why say external?}\sknote{i meant to say that they enable to expose the service/functions to external world outside the kubernetes cluster} 
routing), collects metrics and provides scaling by interacting with the Kubernetes orchestration engine.
%describes the key components of OpenFaaS. It provides t
The API gateway can be scaled to multiple instances.
% \Scut{We can configure the queue size and timeout parameters of the gateway.} 
Also, it can be replaced by a third-party Ingress controller.

% to the container
%It provides an unmanaged and generic interface between the outside world and the serverless function. 
%The Watchdog marshals the HTTP requests from the API Gateway to invoke the serverless function. 
%\knote{this sentence seems unecessary.}
% \Scut{It acts as an init function and forks the process (function) and passes to it the HTTP request via stdin and reads a HTTP response via stdout.}
% %A command line interface is used to package each function into a Docker container. 
% \Scut{Additionally, OpenFaaS provides an AlertManager component (combined with the Prometheus monitor~\cite{Prometheus}) or the Kubernetes Horizontal Pod Autoscaler (HPA) to enable zero-scale and rate based auto-scaling features.}
%The key difference with the OpenFaaS is that any process can become a serverless function through the Watchdog component and a Docker container, thus it allows to run functions coded in any language. %This allows running the function coded in any language without any time/duration constraints. \knote{why, do others have time/duration (do you mean duration of execution?) constraints? Did you say it elsewhere for the other platforms??} 

Each function pod consists of a single container running two kinds of processes namely the i) `of-watchdog' and ii) user deployed function process. The `of-watchdog' is a tiny Golang HTTP server that serves as the entry-point for HTTP requests to be forwarded to the function process. 
% The watchdog component also exports the queue size and timeout configuration parameters. 
% We analyze the performance impact of operating the watchdog in 3 modes:
Based on use case requirements, the `of-watchdog' can be operated in 3 modes, i.e., `HTTP', `streaming' and `serializing'. In `HTTP' mode, the function is forked only once to one instance (worker) at the beginning and kept warm for the entire life-cycle of the function pod. In both the `streaming' and `serializing' mode, a new function instance (worker) is forked for every request, resulting in significant cold-start latency and impact on the throughput.
% Fig.~\ref{fig:of_watchdog_perf_rps} shows the throughput and fig.~\ref{fig:of_watchdog_perf_latency} the latency when running the watchdog in different supported modes.
Fig.~\ref{fig:of_watchdog_perf} shows the throughput and latency when running the watchdog in different supported modes. The `streaming' mode results in very low performance and is typically only desirable for memory-heavy workloads, while the `serializing' mode is equally poor due to fork per request. For our subsequent evaluation, we choose the `HTTP' mode.

%The processing model supports both `at-least once' and `exactly-once' ;  
%\knote{what are these 3 modes? did we explain them?} 
\begin{figure}[htb!]\vspace{-3mm}
\begin{subfigure}{.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{plots/openfaas_of_watchdog_modes_perf_rps-crop.pdf}
    \vspace{-5mm}
    \caption{Throughput in requests/second.}
    \label{fig:of_watchdog_perf_rps}
\end{subfigure}%
\begin{subfigure}{.5\columnwidth}
    \centering
    \vspace{1mm}
    \includegraphics[width=\linewidth]{plots/openfaas_of_watchdog_modes_perf_cdf-crop.pdf}
    \vspace{-5mm}
    \caption{Latency in ms.}
    \label{fig:of_watchdog_perf_latency}
\end{subfigure}%
\vspace{-4mm}
\caption{Throughput and latency for different modes of OpenFaaS of-watchdog (100 concurrent requests).}
\label{fig:of_watchdog_perf}
\vspace{-4mm}
\end{figure}


\noindent{\bf Knative}:
%\vspace{-1mm}\subsubsection{Knative}\vspace{-1mm}
\Scut{
The Knative builds on top of Kubernetes~\cite{burns2016borg} %and Istio\~cite{istio}, 
to provide container based runtime for deploying  serverless applications. %with advanced network routing.
\Scut{Knative provides a set of building blocks for serverless functions that can be run on top of Kubernetes.}%\knote{can you say something about who supports it, and what it is particularly good for?}\sknote{yes, will do.}  
%It was created originally by Google with contributions from over 50 different companies~\cite{knative_about}. 
Knative, by default provides the Istio\footnote{\url{https://istio.io}} ingress controller, but, it can also be plugged with other third party ingress controllers.
%delivers an essential set of components to build and run serverless applications on Kubernetes
The distinct feature of Knative is the `panic mode' scaling mechanism of the autoscaler component. %, which supports two modes of operation namely the stable and panic mode. 
Panic mode enables the autoscaler to be more responsive to sudden traffic spikes (two times the desired average traffic or a configured threshold value) by quickly scaling the functions instances (up to $10\times$ the current pod count or the maximum configured limit). 

\Scut{Knative has three main components: i) Build, ii) Serving and iii) Eventing. 
The Build component is implemented using a Kubernetes CRD and is a pluggable model for building applications (in containers) from source code. 
The Serving component extends Kubernetes to provide runtime computing support for deploying and running serverless workloads. This component also includes the `autoscaler' pod, and provides autoscaling feature including the scale-to-zero support based on received requests. 
The Eventing component provides the necessary primitives for consuming and producing events.}
%From
}
Fig.~\ref{fig:knative_arch}, shows the key components of Knative.
We see that each function pod consists of two containers namely the `queue-proxy' and the `function'. The `queue-proxy' is responsible for queuing incoming requests and forwarding them to the `function' container for execution. It also handles the timeout of queued requests. This queue enables the worker to quickly fetch requests from the ingress controller and process them, thus achieving better throughput, although incurring queuing latency.
Interestingly, we can observe that since Knative implements the `queue-proxy' and `function' as two different containers in a pod, the communication overhead is higher than the process model of the Nuclio and OpenFaaS, resulting in relatively lower performance. %This results in relatively lower performance %(lower throughput and higher latency) 
%than Nuclio and OpenFaaS.
%\vspace{-3mm}
\begin{figure}[htb!]\vspace{-4mm}
\begin{subfigure}{.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{plots/knative_worker_perf_rps-crop.pdf}
    \vspace{-6mm}
    \caption{Throughput in requests/second.}
    \label{fig:knative_worker_perf}
\end{subfigure}%
\begin{subfigure}{.5\columnwidth}
    \centering
    \vspace{1mm}
    \includegraphics[width=\linewidth]{plots/knative_worker_perf_cdf-crop.pdf}
    \vspace{-6mm}
    \caption{Latency in ms.}
    \label{fig:knative_worker_lat}
\end{subfigure}%
\vspace{-4mm}
\caption{Throughput and latency for different number of workers within one Knative function pod (100 concurrent requests).}
\vspace{-4mm}
\label{fig:knative_worker}
\end{figure}

\vspace{1mm}
For the python runtime, we observed that Knative levarages gunicorn\footnote{\url{http://gunicorn.org}} - a Python web server gateway interface (WSGI) server, %\knote{for a HTTP server?? There is something wrong with this sentence}
which supports the pre-fork worker model to create multiple worker processes in a function pod. However, unlike Nuclio, the number of concurrent workers is not exported as a configuration parameter for deployment. 
Figure~\ref{fig:knative_worker} shows the impact on throughput and latency for multiple workers. The characteristics are similar to the Nuclio workers, discussed earlier.% (\S\ref{ssec:nuclio}).

Another distinct feature of Knative is the `panic mode' scaling mechanism of the autoscaler component. %, which supports two modes of operation namely the stable and panic mode. 
Panic mode enables the autoscaler to be more responsive to sudden traffic spikes (two times the desired average traffic or a configured threshold value) by quickly scaling the functions instances (up to $10\times$ the current pod count or the maximum configured limit).

\noindent{\bf Kubeless}:
%\subsubsection{Kubeless}
Kubeless is another open source platform built on top of Kubernetes\Scut{, based on the three basic primitives: functions, triggers and runtime. 
A function is a representation of the code to be executed, and trigger is an event source. 
A trigger can be associated with a single function or to a group of functions depending on the event source type.
A runtime represents a language and runtime specific environment in which a function will be executed}.
%The main component of this platform is a CRD controller that continuously watches for changes to function objects and takes the necessary actions, such as creation or deletion of a new function object. The runtime image used to deploy a function can be explicitly specified by the user, the image artifact is generate on-the-fly, or a pre-built image is used where using Kubernetes’ configmap the function code is deployed into the corresponding Kubernetes pod. Upon deletion, the controller releases the used computing resources. %Figure~\ref{fig:kubeless_arch} describes the key components and the working model of serverless functions in Kubeless. Kubeless ensures that the associated function(s) are invoked at least once. 
Figure~\ref{fig:kubeless_arch} describes the key components and the working model of serverless functions in Kubeless. 
%We chose the Traefik\footnote{\url{https://traefik.io}} as the ingress controller.
We also experimented with NGINX ingress controller,\footnote{\url{https://kubernetes.github.io/ingress-nginx}} and %eventually 
opted for Traefik due to better performance.%\footnote{\url{https://traefik.io}} 
%Kubeless ensures that the associated function(s) are invoked at least once.
%\knote{why are we bringing up at least once here??}\sknote{commented it.. not have much to write about Kubeless.} 

%\input{src/ServerlessPlatforms.tex}


\vspace{-1mm}\subsubsection{Exporting Services and Network routing}\vspace{-1mm}
%All of these discussed 
Serverless frameworks leverage Kubernetes network model to export services (cluster of function pods) and to route requests to specific functions. An API Gateway and/or the Ingress Controller components of the serverless platform can be either exported with a public IP address or can also use the Kubernetes networking model to export the services. 
% overlay based Kubernetes networking framework
Fig.~\ref{fig:svc_export_flannel_arch} describes `Flannel' - a simple Kubernetes overlay networking framework to export serverless functions and route the traffic to function pods. 
% using Kubernetes services. 
% (listen to traffic for the virtual Kubernetes cluster IP range)
% the routing and
The Kube-Proxy component of Kubernetes is responsible for setting up the routing and load-balancing rules (\eg setup the netfilter rules to intercept network packets and change their destination/routing) of the traffic intended for Kubernetes pods, while the Kube-Flannel pod is responsible for intercepting the packets destined for Kubernetes pods (listen to traffic for the virtual Kubernetes pod IP range) and performing UDP encapsulation/decapsulation for the traffic exiting/entering the physical network interface.  %Kube-proxy can be operated in one of the three modes: userspace, iptables, or IPVS.
% we show that Flannel (port based overlay) is used to route packets that reach the Kubernetes master node to the specific service function pod.
In Fig.~\ref{fig:svc_export_flannel_arch}, once the API Gateway/Ingress Controller receives client packets, and determines the service (function) to be executed, it leverages the Kube-Proxy and Kube-Flannel to load-balance and route the traffic to a specific function pod of a worker node. With Kube-Flannel, the traffic leaving the physical network interface is encapsulated and carried over an unreliable UDP transport. 


\noindent \textbf{Impact of Ingress Controller and API Gateway components:}
Typically, the API Gateway components enable the URL based routing to different services in a Kubernetes cluster. The function pods are dynamic entities that can be created and destroyed any time because of zero-scaling, auto-scaling, failures \etc Hence, Kubernetes provides service (a virtual cluster with fixed IP, \textsl{a.k.a.} `Cluster IP') as an abstraction to access the pods of a similar kind. 
The API Gateway/Ingress controllers can route the incoming requests in two possible ways: i) route the incoming traffic to the service and let Kubernetes control load-balancing of the traffic across active pods (\eg with the OpenFaaS API Gateway); ii) load-balance and route the traffic directly to any of the active pod instances (\eg with the Knative-Istio ingress controller).

%  are setup

In the former case (API Gateway), we observed that, in order to avoid the overhead of connection setup time, the API Gateway (OpenFaaS API Gateway) sets up multiple connections with the service `Cluster IP'\footnote{Service being a logical entity, the actual TCP connections are setup with different active pods based on the %network (netfilter) rules setup by Kubernetes.
Kubernetes routing/load-balancing rules (\eg netfilter rules).} at the beginning (the first access to the function) and it uses these connections to forward %relay the
subsequent requests. No new connections are setup afterwards, unless the existing connections get terminated.
Note that if the connections are not setup after auto-scaling, the traffic cannot get distributed to the newly created pods, thus significantly impacting the performance with auto-scaling (refer \S\ref{eval:autoscaling}). %\S\ref{eval:auto:issue} %This significantly impacts load-balancing during the auto-scaling (refer \S\ref{eval:autoscaling}). 
However, in the second case (case ii), the ingress controller needs to keep track of the health and status of all the active pods and setup the connections explicitly with each of the active pods to load-balance the traffic.

==> Serverless_measurement-12 copy/src/ServerlessPlatformDiagrams.tex <==
\begin{figure*}
	\centering
	\begin{subfigure}{.475\textwidth}
	%\begin{subfigure}{.565\textwidth}
		\includegraphics[width=\linewidth]{figures/Nuclio.pdf}
		\vspace{-5mm}
		\caption{Nuclio Serverless Platform}
                \label{fig:nuclio_arch}
	\end{subfigure}%
%\\
	\hspace{2mm}
	%\begin{subfigure}{.58\textwidth}
	\begin{subfigure}{.475\textwidth}
		\includegraphics[width=\linewidth]{figures/OpenFaas.pdf}
		\vspace{-5mm}
		\caption{OpenFaas Serverless Platform}
                \label{fig:openfaas_arch}
	\end{subfigure}
	%\vspace{-2mm}
	%\caption{Working of different kubernetes based serverless platforms.}
%\end{figure*}

%\vspace{-50mm}
%\begin{figure*}
	\centering
	\begin{subfigure}{.475\textwidth}
	%\begin{subfigure}{.565\textwidth}
		\includegraphics[width=\linewidth]{figures/Knative.pdf}
		\vspace{-5mm}
		\caption{Knative Serverless Platform}
                \label{fig:knative_arch}
	\end{subfigure}%
%\\
	\hspace{2mm}
	%\begin{subfigure}{.58\textwidth}
	\begin{subfigure}{.475\textwidth}
		\includegraphics[width=\linewidth]{figures/Kubeless.pdf}
		\vspace{-5mm}
		\caption{Kubeless Serverless Platform}
                \label{fig:kubeless_arch}
	\end{subfigure}
	\vspace{-4mm}
	\caption{Working model for different kubernetes-based serverless platforms (Nuclio, OpenFaas, Knative and Kubeless).}\label{fig:serverless_platforms_arch}
	\vspace{-4mm}
\end{figure*}




==> Serverless_measurement-12 copy/src/ServerlessRouting.tex <==
\Scut{
\begin{figure*}[]\vspace{-3mm}%{.475\textwidth}
	\centering
		\centering
	\begin{subfigure}{.475\textwidth}
	%\begin{subfigure}{.565\textwidth}
		\includegraphics[width=\linewidth]{figures/Kubernetes.pdf}
		\vspace{-5mm}
		\caption{Kubernetes Services used by Serverless Frameworks}
                \label{fig:kubernets_svcs}
	\end{subfigure}%
%\\
	\hspace{2mm}
	%\begin{subfigure}{.58\textwidth}
	\begin{subfigure}{.475\textwidth}
	\includegraphics[width=\textwidth]{figures/Kubernetes_Network_Routing_Flannel.pdf}
	\vspace{-5mm}
	\caption{Kubernetes: Network routing (Flannel mode) to export the services.}
    \label{fig:svc_export_flannel_arch}
    \end{subfigure}
\vspace{-3mm}
\caption{Kubernetes architecture.}
\vspace{-4mm}
\end{figure*}
}

\begin{figure}[]%\vspace{-3mm}%{.475\textwidth}
	\centering
	%\begin{subfigure}{\columnwidth}
	\includegraphics[width=\columnwidth]{figures/Kubernetes_Network_Routing_Flannel3.pdf}
	\vspace{-8mm}
	%\caption{Kubernetes: Network routing (Flannel mode) to export the services.}
	\caption{Kubernetes: Network routing to export the services.}
    \label{fig:svc_export_flannel_arch}
    %\end{subfigure}
\vspace{-4mm}
%\caption{Kubernetes architecture.}
%\vspace{-4mm}
\end{figure}

==> Serverless_measurement-12 copy/src/backup.tex <==
\hide{
% https://theburningmonk.com/2019/04/comparing-nuclio-and-aws-lambda/

With serverless, you delegate the responsibility of running your infrastructure to a platform provider as much as possible. This frees your engineers to focus on building what your customers want from you—the features that differentiate your business from your competitors’. For this philosophy to work, however, the platform needs to not only give you the tools to build those features, but also deliver the performance that will keep engineers satisfied.

Yes, services such as AWS Lambda are powerful, but they have a number of well-documented limitations that make them unsuitable for some workloads. These include: 

\begin{enumerate}
    \item Cold starts and high latency make them unsuitable for real-time applications that require consistent and millisecond-level response times.
    
    \item The pay-per-invocation model makes them costly in high throughput scenarios.
    
    \item The event-driven model, coupled with a max execution time or data size restrictions, makes them unsuitable for long-running tasks or heavy data or AI processing.
    
    \item They are limited to triggers and event sources that are specific to the cloud provider.

\end{enumerate}





Nuclio, an open source serverless platform that is built on top of Kubernetes and comes in both managed platform-as-a-service (PaaS) and self-hosted flavors. In this post, we will compare Nuclio with AWS Lambda, see how Nuclio addresses the above limitations and explore the new use cases Nuclio is unlocking, such as:

\begin{itemize}
    \item High throughput data processing pipelines or ETL.
    \item Serving machine learning models in real time.
    \item Real-time applications such as multiplayer games.
    \item Long-running jobs and services.
\end{itemize}
}


\hide{
%https://hackernoon.com/serverless-and-open-source-where-do-we-stand-today-dff8aec67026


}


\hide{
\section{Related work}
Mohanty et al. [18] performed a feature comparison of four open source serverless frameworks (Kubless, OpenFaaS, Fission, and OpenWhisk). The authors also evaluated the performance of three frameworks (excluding OpenWhisk) when deployed on Kubernetes cluster. In another study, Kritikos et al. [19] reviewed and provided a feature analysis comparison of seven open source serverless frame- works and outlined a set of challenges that require attention from research community. These works have not considered open source frameworks in the context of edge computing.

A number of works have investigated using the serverless computing technology at the edge for executing data process- ing functions. These works have identified the challenge of auto-scaling, which is not predictable to the user. When a function is scaled down, the cold start problem can cause latency issues in a constrained environment [10], [47]–[49].

Serverless computing is receiving increasing attention in the academia [2, 7, 10, 43, 44]. Baldini et al. [2] summarize the general features of serverless platforms and describe open research problems in this area. Lynn et al. [10] present a feature analysis of seven enterprise serverless computing plat- forms, including AWS Lambda, Microsoft Azure Functions, Google Cloud Functions and OpenWhisk. Lee et al. [11] evaluate the performance of public serverless platforms by invoking CPU, memory and disk-intensive functions. They find that AWS Lambda outperforms other public cloud solu- tions. Furthermore, the authors highlight the cost-effectiveness of running functions on serverless platforms as compared to running them on traditional VMs. The authors also present a feature comparison of the public serverless platforms. Lloyd et al. [44] investigate the performance of functions deployed on AWS Lambda and Microsoft Azure Functions. They focus on the impact of infrastructure provisioning on public cloud platforms and identify variations in the functions’ performance depending on the state (cold or warm) of the underlying VM or container. McGrath and Brenner [45] develop a prototype serverless platform implemented in .NET and using Windows containers for executing functions. The authors compare the performance of their prototype platform to AWS Lambda, Google Cloud Functions, Azure Functions and OpenWhisk. Shillaker [43] evaluates the response latency on OpenWhisk at different levels of throughput and concurrent functions. The author identifies research directions for improving start up time in serverless frameworks by replacing containers with a new isolation mechanism in the runtime itself. However, none of the works specifically address open source serverless platforms (Fission, Kubeless, OpenFaaS).

Many serverless application developers have conducted their own experiments to measure coldstart latency, function instance lifetime, maximum idle time before shut down, and CPU usage in AWS Lambda [10–12, 19, 27, 28, 40]. Unfortunately, their experiments were ad-hoc, and the results may be misleading because they did not control for contention by other instances. A few research papers report on measured performance in AWS. Hendrickson et al. [18] measured request latency and found it had higher latency than AWS Elastic Beanstalk (a platform-as-a-service system). McGrath et al. [34] conducted preliminary measurements on four serverless platforms, and found that AWS achieved better scalability, coldstart latency, and throughput than Azure and Google. A concurrent study from Lloyd et al. [33] investigated the factors that affect application performance in AWS and Azure. The authors developed a heuristic to identify the VM a function runs on in AWS based on the VM uptime in /proc/stat. Our experimental evaluation suggests that their heuristic is unreliable (see §4.5), and that the conclusions they made using it are mostly inaccurate.
}

==> Serverless_measurement-12 copy/src/my_packages.tex <==
%\setlength{\textfloatsep}{10pt plus 1.0pt minus 2.0pt}
%\setlength{\intextsep}{10pt plus 2pt minus 2pt}

%\usepackage{usenix,epsfig,endnotes}
%\usepackage{usenix,epsfig}
\usepackage{booktabs}
\usepackage{outlines}
\usepackage{epsfig}
\usepackage{graphicx}
%\usepackage[sort]{cite}  %resulting into errors with new ACM format.
%\usepackage[numbers,sort&compress]{natbib}

\PassOptionsToPackage{hyphens}{url}
\usepackage[hyphens]{url}
%To keep the foot notes in the footer
\usepackage[bottom,para]{footmisc}
\usepackage{multirow}
%\usepackage[demo]{graphicx}
\usepackage{caption}
\usepackage{xspace} %\xspace
\usepackage{lipsum}
\usepackage{subcaption}
\usepackage{amsfonts} % \checkmark
%\usepackage{subfig}
\DeclareGraphicsExtensions{.png, .pdf, .jpg, .bmp}

\usepackage{filecontents}
\usepackage{tikz}
\usepackage{amsmath}

\usepackage{graphicx}
\usepackage{tabularx}
\usepackage{multirow}
%\usepackage{multicol}
\usepackage{balance}
%\usepackage{microtype}
\usepackage{makecell}
\usepackage{adjustbox}

 
\usepackage{tcolorbox}
%\usepackage[font=small,skip=4pt]{caption}
%\usepackage[compact]{titlesec}
%\titlespacing*\section{0pt}{2.5ex}{1ex}
%\titlespacing*\subsection{0pt}{1.5ex}{0.5ex}
%\titlespacing*\subsubsection{0pt}{1ex}{0.5ex}

\usepackage{enumitem}
\setlist{topsep=1pt,itemsep=1pt,parsep=1pt,itemindent=0pt,leftmargin=0.13in}
\usepackage{outlines}

%Highlite capability
\usepackage{soul}
\soulregister\cite7
\soulregister\ref7

%For change Tracking
\usepackage{changes}

\newcommand{\name}{OpenSLXXX\xspace}
\newcommand{\System}{OpenSLXXX\xspace}
\newcommand{\manager}{OpenSLXXX\xspace}
\newcommand{\libnf}{{\em libnf}\xspace}
\newcommand{\nflib}{{\em libnf}\xspace}
\newcommand{\ie}{{\em i.e., \/}}
\newcommand{\eg}{{\em e.g., \/}}
\newcommand{\etc}{{\em etc. \/}}
\newcommand{\etal}{{\em et al.\/}}
\newcommand{\hide}[1] {}
\newcommand{\head}[1]{\vspace{1mm}\noindent{\bf #1}}
\renewcommand{\head}[1]{\vspace{1mm}\noindent{\it #1}}
% \renewcommand{\head}[1]{\vspace{1mm}\noindent{#1}}
\newcommand{\headbf}[1]{\vspace{1mm}\noindent{\bf #1}}

\newcommand{\note}[1]{{\color{red}[#1]}}
\renewcommand\_{\textunderscore\allowbreak}
\newcommand{\mnote}[1]{{$\langle${\textcolor{red}{MA: \textbf{#1}}}$\rangle$}}
\newcommand{\twnote}[1]{{\color{red}[TW: #1]}}
\newcommand{\kknote}[1]{{\color{red}[KK: #1]}}
\newcommand{\knote}[1]{{\color{red}[KK: #1]}}
\newcommand{\srnote}[1]{{\color{red}[SR: #1]}}
\newcommand{\jwnote}[1]{{\color{red}[JW: #1]}}
\newcommand{\sknote}[1]{{\color{magenta}[SK: #1]}}
\newcommand{\revisit}[1]{{\color{cyan}Check: #1}}
\newcommand{\findcite}[1]{\textcolor{magenta}{$^\text{[}$\footnote{\textcolor{red}{Find citation: #1}}$^\text{]}$}}
\newcommand{\refine}[1]{\textcolor{blue}{[{\bf REFINE:} #1]}}
\newcommand{\newtext}[1]{{\color{red} \hl{NewText: #1}}}
%\newcommand{\trackchange}[1]{\textcolor{blue}{#1}}


\renewcommand{\mnote}[1]{\hide{{$\langle${\textcolor{blue}{MA: \textbf{#1}}}$\rangle$}}}
%\renewcommand{\twnote}[1]{\hide{{\color{red}[TW: #1]}}}
%\renewcommand{\kknote}[1]{\hide{{\color{red}[KK: #1]}}}
\renewcommand{\knote}[1]{\hide{{\color{red}[KK: #1]}}}
%\renewcommand{\srnote}[1]{\hide{{\color{red}[SR: #1]}}}
%\renewcommand{\jwnote}[1]{\hide{{\color{red}[JW: #1]}}}
\renewcommand{\sknote}[1]{\hide{{\color{magenta}[SK: #1]}}}


\newcommand{\trackchange}[1]{\textcolor{blue}{#1}}
%\newcommand{\trackupdate}[1]{\textcolor{magenta}{{\bf} #1}}
\newcommand{\trackupdate}[1]{\textcolor{magenta}{#1}}
\newcommand{\trackupdates}[1]{\textcolor{green}{#1}}

% before submission, please uncomment the following commands
% \renewcommand{\trackchange}[1]{{#1}}
% \renewcommand{\trackupdate}[1]{{#1}}
% \renewcommand{\trackupdates}[1]{{#1}}

%Change the footnote to endnote.
%\renewcommand{\footnote}[1]{\endnote{#1}}

% Fix to reclaim the copyright space
%\makeatletter
%\def\@copyrightspace{\relax}
%\makeatother

\usepackage{booktabs} % For formal tables
\usepackage{listings}
\usepackage{color}

% % for page num
% \usepackage{fancyhdr}
% \usepackage{lipsum}
% \usepackage{lastpage}

% for beautiful url
\usepackage{url}
%\usepackage{breakurl}
%\usepackage[breaklinks]{hyperref}
% \def\UrlBreaks{\do\/\do-}

\definecolor{dkgreen}{rgb}{0,0.6,0}
\definecolor{gray}{rgb}{0.5,0.5,0.5}
\definecolor{mauve}{rgb}{0.58,0,0.82}

\lstset{frame=tb,
	language=C,
	aboveskip=3mm,
	belowskip=3mm,
	showstringspaces=false,
	columns=flexible,
	basicstyle={\small\ttfamily},
	numbers=none,
	numberstyle=\tiny\color{gray},
	keywordstyle=\color{blue},
	commentstyle=\color{dkgreen},
	stringstyle=\color{mauve},
	breaklines=true,
	breakatwhitespace=true,
	tabsize=3
}
%\usepackage{enumerate}

% \usepackage{floatrow}
% Table float box with bottom caption, box width adjusted to content
% \newfloatcommand{capbtabbox}{table}[][\FBwidth]

\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}

\newcommand{\Scut}[1] {}
\newcommand{\Sshow}[1] {#1}

==> Serverless_measurement-12 copy/src/pending_items.tex <==
Useful comments:
1. Graphs: 
(1) Bold figure captions; 
(2) Enlarge figures; 
(3) Use a log scale on the y-axis of Fig 6(a) and Fig 8(a) to make the Kubeless data more readable;
2. Experiments: 
(1) Explain where is the client and why the client is not the bottleneck; 
(2) Explain why the parameters of auto-scaling experiments are chosen;
3. Background and comparison:
(1) Since we need to enlarge figures and add the explanation in evaluation section, we need to simplify the background section to make sure to fit the final version to 6 pages;
(2) Working model figure (Fig.2): draw a single generic model and illustrate the similarities and differences of four platforms (with an extra summary table);
4. Overall:
(1) Add more insights;
(2) Add the discussion on other aspects, such as the different strategies to multiplex and their implications/tradeoff to security (sharing among several distrustful functions) [Maybe do it later.];

Ignored comments:
1. Graphs: 
(1) convert scientific notation to actual values on y-axis [Reason: the actual values are too big to be directly shown in the figure]; 
2. Overall
Update the title: to mention kubernetes. Maybe change to "Understanding Kubernetes-based Open Source Serverless Platforms: Design Considerations and Performance";

Other pending items:
1. Experiments:
(1) Explain the reason of long tail of Kubeless and OpenFaaS in latency CDF figures;
(2) Find the more exact payload threshold of openfaas (http and streaming mode) and kubeless, and explain why the throughput drops dramatically after the threshold;
(3) Update the auto-scaling experiment with bursty workload: send a fix number of requests in one shot and records the metrics;

==> plots/eval1_plots.tex <==
\hide{
\begin{figure*}[htb!]
\begin{subfigure}{.5\textwidth}
    \centering
    \includegraphics[width=3.2in, trim=0.01cm 0.01cm 0.01cm 0.01cm, clip=true]{plots/access_mode_rps_barplot.pdf}
    \vspace{-3mm}
    \caption{Throughput in requests/second.}
    \label{fig:ThroughputDiffModes}
    % \vspace{-4mm}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
	\centering
	\includegraphics[width=3.4in, trim=0.01cm 0.01cm 0.01cm 0.01cm, clip=true]{plots/boxplot_configuration.pdf}
    \vspace{-3mm}
    \caption{Latency in ms.}
    \label{fig:LatencyDiffModes}
    \vspace{-6mm}
\end{subfigure}
\caption{Throughput and latency for different methods of exporting the services for different serverless platforms.}
\label{fig:DiffModes}
\end{figure*}
}
\hide{
\begin{figure}[htb!]
\begin{subfigure}{.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth, trim=0.01cm 0.01cm 0.01cm 0.01cm, clip=true]{plots/access_mode_rps_barplot.pdf}
    \vspace{-6mm}
    \caption{Throughput in requests/second.}
    \label{fig:ThroughputDiffModes}
    % \vspace{-4mm}
\end{subfigure}
\begin{subfigure}{.5\columnwidth}
	\centering
	\includegraphics[width=\linewidth, trim=0.01cm 0.01cm 0.01cm 0.01cm, clip=true]{plots/boxplot_configuration.pdf}
    \vspace{-6mm}
    \caption{Latency in ms.}
    \label{fig:LatencyDiffModes}
\end{subfigure}
\vspace{-4mm}
\caption{Throughput and latency for different methods of exporting the services for different serverless platforms.}
\label{fig:DiffModes}
\end{figure}

\begin{figure}[htb!]
\begin{subfigure}{.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth, trim=0.01cm 0.01cm 0.01cm 0.01cm, clip=true]{plots/http_payload_rps_barplot.pdf}
    \vspace{-5mm}
    \caption{Throughput in requests/second.}
    \label{fig:ThroughputPayload}
    % \vspace{-4mm}
\end{subfigure}
\begin{subfigure}{.5\columnwidth}
	\centering
	\includegraphics[width=\linewidth, trim=0.01cm 0.01cm 0.01cm 0.01cm, clip=true]{plots/http_payload_latency_cdf.pdf}
    \vspace{-5mm}
    \caption{CDF of Latency.}
    \label{fig:LatencyPayload}
\end{subfigure}
\vspace{-3mm}
\caption{Throughput and latency of different payload sizes for different serverless platforms.}
\label{fig:DiffPayload}
\end{figure}
}

==> src/Discussion.tex <==
Some of the aspects surrounding the open-source serverless platforms that need additional community attention. 
\begin{itemize}
    \item 
    \item Flexibility vs learning time:
    \item Reliance on Kubernetes services and auto-scaling: Pros and cons
    \item Need for 'rate-cost' proportional scheduling and scaling of services.
    \item Debug and Support service for open-source platforms:
\end{itemize}

==> src/backup.tex <==
\hide{
% https://theburningmonk.com/2019/04/comparing-nuclio-and-aws-lambda/

With serverless, you delegate the responsibility of running your infrastructure to a platform provider as much as possible. This frees your engineers to focus on building what your customers want from you—the features that differentiate your business from your competitors’. For this philosophy to work, however, the platform needs to not only give you the tools to build those features, but also deliver the performance that will keep engineers satisfied.

Yes, services such as AWS Lambda are powerful, but they have a number of well-documented limitations that make them unsuitable for some workloads. These include: 

\begin{enumerate}
    \item Cold starts and high latency make them unsuitable for real-time applications that require consistent and millisecond-level response times.
    
    \item The pay-per-invocation model makes them costly in high throughput scenarios.
    
    \item The event-driven model, coupled with a max execution time or data size restrictions, makes them unsuitable for long-running tasks or heavy data or AI processing.
    
    \item They are limited to triggers and event sources that are specific to the cloud provider.

\end{enumerate}





Nuclio, an open source serverless platform that is built on top of Kubernetes and comes in both managed platform-as-a-service (PaaS) and self-hosted flavors. In this post, we will compare Nuclio with AWS Lambda, see how Nuclio addresses the above limitations and explore the new use cases Nuclio is unlocking, such as:

\begin{itemize}
    \item High throughput data processing pipelines or ETL.
    \item Serving machine learning models in real time.
    \item Real-time applications such as multiplayer games.
    \item Long-running jobs and services.
\end{itemize}
}


\hide{
%https://hackernoon.com/serverless-and-open-source-where-do-we-stand-today-dff8aec67026


}


\hide{
\section{Related work}
Mohanty et al. [18] performed a feature comparison of four open source serverless frameworks (Kubless, OpenFaaS, Fission, and OpenWhisk). The authors also evaluated the performance of three frameworks (excluding OpenWhisk) when deployed on Kubernetes cluster. In another study, Kritikos et al. [19] reviewed and provided a feature analysis comparison of seven open source serverless frame- works and outlined a set of challenges that require attention from research community. These works have not considered open source frameworks in the context of edge computing.

A number of works have investigated using the serverless computing technology at the edge for executing data process- ing functions. These works have identified the challenge of auto-scaling, which is not predictable to the user. When a function is scaled down, the cold start problem can cause latency issues in a constrained environment [10], [47]–[49].

Serverless computing is receiving increasing attention in the academia [2, 7, 10, 43, 44]. Baldini et al. [2] summarize the general features of serverless platforms and describe open research problems in this area. Lynn et al. [10] present a feature analysis of seven enterprise serverless computing plat- forms, including AWS Lambda, Microsoft Azure Functions, Google Cloud Functions and OpenWhisk. Lee et al. [11] evaluate the performance of public serverless platforms by invoking CPU, memory and disk-intensive functions. They find that AWS Lambda outperforms other public cloud solu- tions. Furthermore, the authors highlight the cost-effectiveness of running functions on serverless platforms as compared to running them on traditional VMs. The authors also present a feature comparison of the public serverless platforms. Lloyd et al. [44] investigate the performance of functions deployed on AWS Lambda and Microsoft Azure Functions. They focus on the impact of infrastructure provisioning on public cloud platforms and identify variations in the functions’ performance depending on the state (cold or warm) of the underlying VM or container. McGrath and Brenner [45] develop a prototype serverless platform implemented in .NET and using Windows containers for executing functions. The authors compare the performance of their prototype platform to AWS Lambda, Google Cloud Functions, Azure Functions and OpenWhisk. Shillaker [43] evaluates the response latency on OpenWhisk at different levels of throughput and concurrent functions. The author identifies research directions for improving start up time in serverless frameworks by replacing containers with a new isolation mechanism in the runtime itself. However, none of the works specifically address open source serverless platforms (Fission, Kubeless, OpenFaaS).

Many serverless application developers have conducted their own experiments to measure coldstart latency, function instance lifetime, maximum idle time before shut down, and CPU usage in AWS Lambda [10–12, 19, 27, 28, 40]. Unfortunately, their experiments were ad-hoc, and the results may be misleading because they did not control for contention by other instances. A few research papers report on measured performance in AWS. Hendrickson et al. [18] measured request latency and found it had higher latency than AWS Elastic Beanstalk (a platform-as-a-service system). McGrath et al. [34] conducted preliminary measurements on four serverless platforms, and found that AWS achieved better scalability, coldstart latency, and throughput than Azure and Google. A concurrent study from Lloyd et al. [33] investigated the factors that affect application performance in AWS and Azure. The authors developed a heuristic to identify the VM a function runs on in AWS based on the VM uptime in /proc/stat. Our experimental evaluation suggests that their heuristic is unreliable (see §4.5), and that the conclusions they made using it are mostly inaccurate.
}

==> src/pending_items.tex <==
Useful comments:
1. Graphs: 
(1) Bold figure captions; 
(2) Enlarge figures; 
(3) Use a log scale on the y-axis of Fig 6(a) and Fig 8(a) to make the Kubeless data more readable;
2. Experiments: 
(1) Explain where is the client and why the client is not the bottleneck; 
(2) Explain why the parameters of auto-scaling experiments are chosen;
3. Background and comparison:
(1) Since we need to enlarge figures and add the explanation in evaluation section, we need to simplify the background section to make sure to fit the final version to 6 pages;
(2) Working model figure (Fig.2): draw a single generic model and illustrate the similarities and differences of four platforms (with an extra summary table);
4. Overall:
(1) Add more insights;
(2) Add the discussion on other aspects, such as the different strategies to multiplex and their implications/tradeoff to security (sharing among several distrustful functions) [Maybe do it later.];

Ignored comments:
1. Graphs: 
(1) convert scientific notation to actual values on y-axis [Reason: the actual values are too big to be directly shown in the figure]; 
2. Overall
Update the title: to mention kubernetes. Maybe change to "Understanding Kubernetes-based Open Source Serverless Platforms: Design Considerations and Performance";

Other pending items:
1. Experiments:
(1) Explain the reason of long tail of Kubeless and OpenFaaS in latency CDF figures;
(2) Find the more exact payload threshold of openfaas (http and streaming mode) and kubeless, and explain why the throughput drops dramatically after the threshold;
(3) Update the auto-scaling experiment with bursty workload: send a fix number of requests in one shot and records the metrics;
